Multiplayer Multi-armed Bandits for Optimal Assignment in Heterogeneous Networks

We consider an ad hoc network where multiple users access the same set of channels. The channel characteristics are unknown and could be different for each user (heterogeneous). No controller is available to coordinate channel selections by the users, and if multiple users select the same channel, they collide and none of them receive any rate (or reward). For such a completely decentralized network we develop algorithms that aim to achieve optimal network throughput. Due to lack of any direct communication between the users, we allow each user to exchange information by transmitting in a specific pattern and sense such transmissions from others. However, such transmissions and sensing for information exchange do not add to network throughput. For the wideband sensing and narrowband sensing scenarios, we first develop explore-and-commit algorithms that converge to near-optimal allocation with high probability in a small number of rounds. Building on this, we develop an algorithm that gives logarithmic regret, even when the number of users changes with time. We validate our claims through extensive experiments and show that our algorithms perform significantly better than the state-of-the-art CSM-MAB, dE3 and dE3-TS algorithms.

==> FullSensing.tex <==
\subsection{Full sensing}
\label{sec:FullSensing}
In this section we develop an algorithm named  Distributed Optimal Assignment with Full Sensing (DOA-FS). The inputs to the algorithm are $N, K, \epsilon$ and $\delta$ and the algorithm guarantees an $(\epsilon, \delta)$-optimal assignment within a finite number of rounds. The algorithm consists of three phases namely 1) Random Hopping (RH) 2) Sequential Hopping (SH) and 3) Bernoulli Signaling (BS). These phases run sequentially to estimate the matrix $M$. At the end, all players apply the Hungarian method\footnote{Any algorithm that computes the optimal assignment can be used} and play the arm given by the optimal assignment thereafter. The pseudo-code of the algorithm is given in Algorithm (\ref{alg:Algo1}). The algorithm is run by each player separately. We suppress index $n$ to avoid cluttering in the presentation.

\begin{algorithm}[!h]
	\caption{DOA-FS} \label{alg:Algo1}
	\begin{algorithmic}[1]
		\State	Input: {$K, \epsilon, \delta$}
		\State	\textbf{Initial Orthogonal Assignment}: $(N, k,n)= RH(K, \delta)$ 
		\State	 Exploration: $\hat{\mu}_i=SH(a, K, \epsilon,\delta )$ 
		\State  $\hat{M}=SE(N,\hat{\mu}_i, \epsilon, \delta)$
		\State Find  optimal assignment $\hat{\pi}^*$ on $\hat{M}$ 
		\State \textbf{Exploitation}: Play $\hat{\pi}^*(k)$ till end
		%		\State Play arm assigned by it.
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!h]
	\caption*{\textbf{Phase 1:} Random Hopping (RH)}
	\begin{algorithmic}[1]
		\State Input: $K, \delta$  
		\State Initialize: Set $Lock=0$ and Compute $T_{r}$ from (\ref{eqn:RHLen})
		\For{$t=1 \dots T_{r}$}
		\If{($Lock == 1$)}
		\State Select the same arm, $\alpha_t = \alpha_{t-1}$
		\Else
		\State Randomly select a channel, $\alpha_t \sim U([K])$
		\State Set $Lock=1$ if no collision is observed
		\EndIf
		\EndFor	
		\State Find number of players $(N)$ and player index $(n)$
		\State Return $N,n$ and index of current arm $(k)$.
	\end{algorithmic}
\end{algorithm}
% \vspace{-.5cm}
\begin{algorithm}[!h]
	\caption*{\textbf{Phase 2:} Sequential Hopping (RH)}
	\begin{algorithmic}[1]
		\State Input: $K, \delta, \epsilon, k,n$  
		\State Set $\alpha_{T_{r}}=k$, $r_i=0 \;\; \forall i\in [K]$ and compute $T_{s}$ \textcolor{red}{from (\ref{eqn:SHLen})}
		\For{$t=T_{rh}+1 \dots KT_{s}$}
		\State Play arm $\alpha_t=(\alpha_{t-1} +1 )\mod K$
		\State Observe reward $X_{\alpha_t}$ and update $r_{\alpha_t}=r_{\alpha_t} + X_{\alpha_t}$
		\EndFor	
		\State Estimate $\hat{\mu}_{n,k}=r_{k}/T_{sh} \; \forall k \in [K]$
		\State Return $\hat{\mu}_n= \{\hat{\mu}_{n,k}\}$.
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!h]
	\caption*{\textbf{Phase 3:} Bernoulli Signaling (BS)}
	\begin{algorithmic}[1]
		\State Input: $K, \delta, \epsilon, \hat{\mu}_n$  
		\State Set $o_{i,j}=0 \;\forall\; i, j\in [K]$ and compute $T_{b}$ \textcolor{red}{from (\ref{eqn:BSLen})}
		\For{$j=1,2\dots, K$}
		\For {$T_b$ number of rounds}
		\State Transmit with probability $\hat{\mu}_{n,j}$ on current arm
		\State $A=\left \{k\in [K]: \mbox{transmission is sensed on arm } k\right \}$
		\State  Update $o_{i,j}= o_{i,j}+ 1$ for all $i \in A$
		\EndFor
		\EndFor	
		\State Estimate $\widehat{\mu}_{i,j}=o_{i,j}/T_e \; \forall \; i,j \in [K]$
		\State Return $\hat{M}= \left \{\widehat{\mu}_{i,j}\right \}$.
	\end{algorithmic}
\end{algorithm}
The RH phase ensures that all players are on different arms (orthogonalized). During this phase, each player selects an arm uniformly at random in each round till they experience a collision free transmission. Once it happens, they continue to play that arm till the end of RH phase. The length of the RH phase is set such that all players are orthogonalized with high probability.

The SH phase ensures that all the players learn mean rewards they see on the arms. During this phase, all the players select the arms sequentially, i.e., arm $(k+1)\mod K$ is played in the next round after playing arm $k$ in the current round. Since the orthogonal allocation is maintained in each round, no collisions are incurred in this phase. The length of the SH phase is set such that the mean rewards are estimated with high accuracy. 

In the BS phase, each player signals her observation of mean rewards to others and also learns reward seen by others through their signals. This is achieved as follows. The BS phase consists of $K$ frames each of $T_e$ rounds in which each player plays the same arm that she last played in the SE phase. In the $i$th frame each player transmits according to a Bernoulli distribution with the Bernoulli parameter set to the value of their estimated mean on arm $i$. They also detect on which other arms transmissions occured and update the number of transmissions observed on each arms. At the end of $K$th frame, each player computes the mean number of transmissions observed on each arm including the arm on which it transmitted. 

Notice that at the end of the BS phase each player will have the same estimate of the reward matrix $M$. Each players then find optimal assignment on $\hat{M}$ and play it thereafter. The guarantees of DOA-FS is given as follows:

\begin{thm}
	\label{thm:DOA-FS}
	For a given $\epsilon>0, \delta \in (0,1)$ let $T_r, T_s$ and $T_e$ be set as follows
	\begin{equation}
		\label{eqn:RHLen}
		T_{r}=\left \lceil \frac{\log(\delta/3K)}{ \log\left(1-1/4K\right)} \right \rceil 
	\end{equation} 
	\begin{equation}
		\label{eqn:SHLen}
		T_s= \left\lceil \frac{8N^2}{\epsilon^2}\log\left(\frac{6NK}{\delta}\right)\right\rceil
	\end{equation}	
	\begin{equation}
		\label{eqn:BSLen}
		T_b=  \left\lceil \frac{8N^2}{\epsilon^2}\log\left(\frac{6K^2}{\delta}\right)\right\rceil
	\end{equation}	
	Then DOA-FS policy is $(\epsilon, \delta)$-optimal after $T_r+KT_s + KT_b$ number of rounds for any mean reard matrix $M$. 
\end{thm}
The proof of the theorem uses the following lemmas. Their proofs are  are given in the appendix, they are straightforward application of the Hoeffding's concentration inequality \cite{}.
\begin{lemma}
	\label{lma:RHPhase}
	Let $\delta \in (0,1)$. If RH phase is run for  $ T_{r}=\left \lceil \frac{\log(\delta/3K)}{ \log\left(1-1/4K\right)} \right \rceil $ number of rounds then all the players will be orthogonalized with probability at least $1-\delta/3$.  
\end{lemma}  

\begin{lemma}
		\label{lma:SHPhase}
For any given $\delta \in (0,1)$ and $\epsilon>0$ set $T_s = \frac{8N^2}{\epsilon^2}\log\left(\frac{6NK}{\delta}\right)$. Then estimated  mean rewards at the end of the SH phase  are such that $|\mu_{n,k}-\hat{\mu}_{n,k}|\leq \epsilon/4N$ for all $n\in [N], k\in [K]$ with probability at least $1 - \delta/3$.
\end{lemma}

\begin{lemma}
		\label{lma:BSPhase}
	For any given $\delta \in (0,1)$ and $\epsilon>0$ set  $T_b = \frac{8N^2}{\epsilon^2}\log\left(\frac{6K^2}{\delta}\right)$. Let $\hat{\mu}_n$ denote the mean reward vector that player $n\in [N]$ signals. Then estimated  mean rewards matrix $\hat{M}=\left \{\widehat{\mu}_{i,j}\right \}$ at the end of the BS phase will be  such that $|\hat{\mu}_{n,k}-\widehat{\mu}_{n,k}|\leq \epsilon/4N$ for all $n\in [N], k\in [K]$ with probability at least $1 - \delta/3$.
\end{lemma}
\noindent
{\textbf{Proof} of Thm (\ref{thm:DOA-FS}):} If (A) denotes all players orthogonalized in RH phase, (B) denotes all players estimate their mean reward within $\epsilon/4N$ accuracy and (C) denotes all players signal their estimates to others within $\epsilon/4N$ accuracy,  the estimated matrix $\hat{M}$ at each player will be such that $|\hat{M}- M|\leq \epsilon I$ after $T:=T_r + K(T_s+ T_b)$ rounds.  Thm. \ref{thm:ApproxHun} then implies that if all players play the optimal assignment obtained from $\hat{M}$, DOA-FS policy will be $\epsilon$-optimal for all $t > T$. Hence we have
\begin{eqnarray*}
	\lefteqn{\Pr\left \{\mbox{DOA-FS is  $\epsilon$-optimal for}\;\; t > T\right \} }\\
	&\geq& \Pr\{\text{A,B,C holds}\}= 1- \Pr\{\text{any of A,B,C does not hold}\}\\
	&>& 1- 3\delta/3= 1- \delta,
\end{eqnarray*}
where the inequality follows from Lemma (\ref{lma:RHPhase}), (\ref{lma:SHPhase}) and (\ref{lma:BSPhase}). \hfill\IEEEQED
\begin{remark}
Note that mean reward corresponding to player $n$ in $\hat{M}$ is $\widehat{\mu}_n$ and not $\hat{\mu}_n$, i.e., the values players signaled to other players in the BS phase and not what she estimated in the SE phase. This done to ensure that all players have the same $\hat{M}$ so that they find the same optimal assignment.
\end{remark}

\begin{remark}
The performance in the BS phase can be improved by listening only on the arms on which players are transmitting. In this case we can set 
$T_b = \frac{8N^2K}{\epsilon^2}\log\left(\frac{6NK}{\delta}\right)$ and still achieve the same result. We skip the details.
\end{remark}

\subsubsection{Packetized vs Bernoulli Signaling }
In the BS phase of DO-FS, players exchange information within high accuracy via Bernoulli distributions. This can be achieved in multiple ways. One possibility is that each player encodes her estimates and signals the same to other using a certain number of bits. For example, each player can encode her estimates within $\epsilon/4N$ accuracy using $\lceil \log_2 (1/\epsilon N)\rceil$. Then, each player needs $K\lceil \log_2 (1/\epsilon N)\rceil$ bits to encode her estimates of all arms. The players can then transmit on an arm as per the bit sequence of their code-- a transmission corresponds to bit '$1$' and a no transmission corresponds to bit  '$0$'. Since players can sense all the arms, within $K\lceil \log_2 (1/\epsilon N)\rceil$ all players will receive the estimates of other players within $\epsilon/4N$ accuracy. By setting $T_b=K\lceil \log_2 (1/\epsilon N)\rceil$ the result of Thm \ref{thm:DOA-FS} will hold with packetized signaling replacing the Bernoulli signaling.
\\
\subsubsection{Handling Multiple Optimal Allocations}
In the design of DOA-FS we assumed that the optimal allocation computed from $\hat{M}$ will be unique. However, there could exists multiple optimal assignment in some cases. In such cases, it may happen that players find different optimal allocation and two players may get the same arm. We next discuss how we can ensure that all players end up with the same optimal assignment even when there exits multiple optimal allocation on $\hat{M}$. 

On using the Hungarian method implemented as done here [scipy], it returns only one optimal assignment and the same always, as they break ties in case of multiple allocations in a particular manner. Hence when players in a system have communicated their rates, each one will have the same rate matrix and hence evaluate the same assignment. 

When multiple allocations 

\subsection{Partial Sensing}
\label{sec:PartialSensing}

In this subsection we study the case where players can listen or transmit on one arm at a time. This setup is applicable where the players correspond to cheap nodes in a wireless ad hoc networks equipped with a single RF chain.

We present the DOA-PS algorithm (\ref{alg:Algo2}), which is a modification of the DOA-FS algorithm, that accommodates the scenario of single sensing. The inputs to the algorithm are $N$, $K$, $\epsilon$ and $\delta$ and the algorithm guarantees an ($\epsilon$, $\delta$) -optimal assignment within a finite number of rounds.

The assumption here is that a player can only transmit or sense at only one channel in a time slot, thus making single-sensing scenario a "stricter" version of the full-sensing case. This affects only the BS phase as now communicating estimated rates to all other players takes more time. 

The full-sensing system enabled players to listen to multiple channels at the same time and thus infer rates of multiple players at once. But now, when a player communicates her rates on a channel, everyone else would have to listen on that channel to infer that player's rates. 
We propose modifications to both versions of communication algorithms - i)Bernoulli Signalling for Single Sensing (BS\_SS) and ii) Packetised Signalling for Single Sensing(PS\_SS).

Both the DOA-FS and the DOA-PS algorithms have exploration, communication and exploitation phases, in respective order. At the end, all players use the Hungarian Algorithm and play the arm corresponding to the evaluated optimal assignment. The only difference between the algorithms is in the communication phase (step 4 of Algorithm (\ref{alg:Algo1})), where $BS\_SS(N,\hat{\mu}_i, \epsilon, \delta)$ is used to calculate the $\hat{M}$.

\iffalse
\begin{algorithm}[!h]
	\caption{DOA-PS} \label{alg:Algo2}
	\begin{algorithmic}[1]
		\State \textbf{Input}: {$K, \epsilon, \delta$}
		\State \textbf{Initial Orthogonal Allocation}: $(N, k,n)= RH(K, \delta)$ 
		\State \textbf{Exploration phase}:$\hat{\mu}_i=SH(a, K, \epsilon,\delta )$ 
		\State $\hat{M}=BS\_SS(N,\hat{\mu}_i, \epsilon, \delta)$
		\State Find  optimal assignment $\hat{\pi}^*$ on $\hat{M}$ 
		\State \textbf{Exploitation phase}: Play $\hat{\pi}^*(k)$ till end
		%		\State Play arm assigned by it.
	\end{algorithmic}
\end{algorithm}
\fi
This algorithm takes $T_r + KT_s + KNT_b$ time slots to give an $(\epsilon,\delta)$-optimal policy as compared to $T_r + KT_s + KT_b $ time slots for the DOA-FS algorithm, with the extra $N$ factor arising in the last term due to difference in the communication phase. The proof for this is similar to that of theorem (\ref{thm:DOA-FS}).


\begin{algorithm}[!h]
	\caption*{\textbf{Phase 3:} Bernoulli Signaling for Single Sensing Case (BS\_SS)}
	\begin{algorithmic}[1]
		\State Input: $K, \delta, \epsilon, \hat{\mu}_n$  
		\State Set $o_{i,j}=0 \;\forall\; i\in [N], j\in [K]$ and $T_{b}$ 
		\For{$i=1,2\dots, N$}
		
		\For{$j=1,2\dots, K$}
		\For {$T_b$ number of rounds}
		\If{($i==n$)}
		\State Transmit with Bernoulli($\hat{\mu}_{n,j}$) on arm $j$
		\If{Transmission is sensed on arm j}
		\State  Update $o_{i,j}= o_{i,j}+ 1$
		\EndIf
		\EndIf
		\EndFor
		\State Estimate $\widehat{\mu}_{i,j}=o_{i,j}/T_b$ \;
		\EndFor	
		\EndFor
		
		\State Return $\hat{M}= \left \{\widehat{\mu}_{i,j}\right \}$.
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!h]
	\caption*{\textbf{Phase 3:} Packetized Signaling for Single Sensing Case (BS\_SS)}
	\begin{algorithmic}[1]
		\State Input: $K, \delta, \epsilon, \hat{\mu}_n$  
		\State Set $o_{i,j}=0 \;\forall\; i\in [N], j\in [K]$ and $T_{b}$ 
		\For{$i=1,2\dots, N$}
		
		\For{$j=1,2\dots, K$}
		\If{($i==n$)}
		\State $B=Encode(\hat{\mu}_{n,j})$
		\State Transmit $B$ on arm $j$
		\EndIf
		\State Receive $B$
		\State $\widehat{\mu}_{i,j}=Decode(B)$
		\EndFor	
		\EndFor
		
		\State Return $\hat{M}= \left \{\widehat{\mu}_{i,j}\right \}$.
	\end{algorithmic}
\end{algorithm}





==> SingleSensing.tex <==


%\subsubsection{Batch vs Repeated Exploration }
%We emphasize on our algorithm to update estimates of rates when explored over epochs rather than using an increasing exploration time. This enables effective use of previous explorations and averaging over multiple batches giving stable and reliable results. \textbf{ MORE}


